The Fallacy of Minimizing Cumulative Regret in the Sequential Task Setting

Online Reinforcement Learning (RL) is typically framed as the process of minimizing cumulative regret (CR) through interactions with an unknown environment. However, real-world RL applications usually involve a sequence of tasks, and the data collected in the first task is used to warm-start the second task. The performance of the warm-start policy is measured by simple regret (SR). While minimizing both CR and SR is generally a conflicting objective, previous research has shown that in stationary environments, both can be optimized in terms of the duration of the task, $T$. In practice, however, in real-world applications, human-in-the-loop decisions between tasks often results in non-stationarity. For instance, in clinical trials, scientists may adjust target health outcomes between implementations. Our results show that task non-stationarity leads to a more restrictive trade-off between CR and SR. To balance these competing goals, the algorithm must explore excessively, leading to a CR bound worse than the typical optimal rate of $T^{1/2}$. These findings are practically significant, indicating that increased exploration is necessary in non-stationary environments to accommodate task changes, impacting the design of RL algorithms in fields such as healthcare and beyond.

==> sections/sec2_example.tex <==
A main result of this paper is that the trade-off characterized in (\ref{equ:existing_lower}) can be significantly stronger when certain changes present. We motivate this with a contextual bandit, where we only allow the agent to run a context-independent policy in the second task ($\Pi^{(2)} = \{\pi \in \Pi: \pi(a \mid x_1) = \pi(a \mid x_2), \text{ for all } (x_1, x_2) \in \gX\}$), while there is no such constraint for the first task. Consider a two-armed ($a_1$ and $a_2$) contextual bandit with two context $x_1$, $x_2$, and the marginal context distribution $P_x$ is uniform random over $\{x_1, x_2\}$. The mean reward for each context and action pair and the marginal mean reward by averaging over context is given by Figure \ref{fig:simulation}. 

\begin{figure}[hpt]
    \includegraphics[width = 0.22\textwidth]{Figures/mean_reward.pdf}
    \includegraphics[width = 0.22\textwidth]{Figures/CR.pdf}
    \includegraphics[width = 0.22\textwidth]{Figures/SR.pdf}
    \caption{(Left panel) The mean reward for each action-context pair and the marginal mean reward by averaging over contexts. Average cumulative regrets (middle) v.s. simple regret (right) over various time steps. The blue lines are UCB and the green lines are UCB + $0.1$-uniform exploration.}
  \label{fig:simulation}
\end{figure}
 
The optimal policy without policy set constraint is to select $a_1$ at $x_1$ and $a_2$ at $x_2$. The issue with regret minimization in the first task is that the dataset collected by the optimal policy of the contextual bandit lacks visitations in $(x_1, a_2)$ and $(x_2, a_1)$. However, to achieve a low simple regret, it is critical to accurately estimate the mean reward for $(x_2, a_1)$ for small $\epsilon$. Therefore, low visitation in $(x_2, a_1)$ hinders a good policy learning for the simple regret. \textbf{In other words, naively minimizing the cumulative regrets leads to a worse simple regret guarantee.} 
% As we will show later, the trade-off between $\CR$ and $\SR$ becomes $\sqrt{\E[\CR]} \E[\SR] = \tilde{\Omega}(1)$, substantially stronger than (\ref{equ:existing_lower}). If one only cares about the simple regret with a minimax rate of $1/\sqrt{T}$, then the rate of cumulative regrets is $\Omega(T)$.
% The trade-off characterized in (\ref{equ:existing_lower}) can be significantly stronger when certain changes present when evaluating simple regret. For instance, instead of learning a contextual bandit, we only allow the agent to output a context-free policy and the simple regret is evaluated with respect to the best context-free policy. This constraint is motivated by real-world applications, where between two RL implementations, the domain experts may decide that certain context introduces gender bias, and thus should be removed in the future RL deployment for fairness concerns. Consider a two-armed ($a_1$ and $a_2$) contextual bandit with two context $x_1$, $x_2$, and the marginal context distribution $P_x$ is uniform. The mean reward for each context and action pair and the marginal mean reward by averaging over context is given by Figure \ref{fig:simulation}. The optimal policy for CB is to select $a_1$ at $x_1$ and $a_2$ at $x_2$. The issue with regret minimization is that the dataset collected by the optimal policy of the contextual bandit lacks visitations in $(x_1, a_2)$ and $(x_2, a_1)$. However, to achieve a low simple regret, it is critical to accurately estimate the mean reward for $(x_2, a_1)$ for small $\epsilon$. Therefore, low visitation in $(x_2, a_1)$ hinders a good policy learning for the simple regret. \textbf{In other words, naively minimizing the cumulative regrets leads to a worse simple regret guarantee.} As we will show later, the trade-off between $\CR$ and $\SR$ becomes $\sqrt{\E[\CR]} \E[\SR] = \tilde{\Omega}(|\gX||\gA|)$, substantially stronger than (\ref{equ:existing_lower}). If one only cares about the simple regret with a minimax rate of $1/\sqrt{T}$, then the rate of cumulative regrets is $\Omega(T)$.

Simple simulation experiment validates this hypothesis. Figure \ref{fig:simulation} compares the average cumulative regret and the simple regret in the second task by running UCB (Upper Confidence Bound) \citep{auer2002using} algorithm (in blue) and UCB mixed with probability 0.1 random exploration (in green) on the task described above. UCB shows a diminishing average cumulative regret with a constant simple regret for the second task. Mixed with 0.1 random exploration, UCB receives a constant average regret, while the simple regret goes to zero, revealing a strong trade-off between cumulative regrets and simple regret. 

==> sections/sec3_minimax.tex <==
% \ziping{Some notation is missing and I need to fixed them}

A major result of this paper is the more restrictive trade-off between cumulative regret and simple regret. We demonstrate this trade-off through a minimax lower bound under mild conditions on the problem instance set.

% We start by defining a \textit{contextual bandit instance} by $S = (P, \Pi, f)$, made up of three components on the outcome distribution, the policy class, and the reward mapping. We further denote a \textit{problem instance} by $\mS = (S^{(1)}, S^{(2)})$, a pair of instances, where $S^{(1)} = (P, \Pi^{(1)}, f^{(1)})$, $S^{(2)} = (P, \Pi^{(2)}, f^{(2)})$. We denote by $\pi^{\star}_{S}$ the optimal policy of the bandit instance $S$ if there is a unique one. 
% We let $\gS(\mS) \subset \gS$ be the subset of $\gS$ such that any $S' \in \gS(\mS)$ shares the same 
% For an instance set $\gS$ and a given instance $\mS$, we denote by $\gS(\mS)\subset\gS$ the subset of all instances that share the same policy classes and reward mappings $(\Pi^{(1)}, \Pi^{(2)}, f^{(1)}, f^{(2)})$ as $S$, while having different $P$.

Since policy classes and reward mappings are known, we may denote a problem instance by $P$, the unknown outcome distribution, and by $\gP$ the set of outcome distributions of interest.

\begin{defn}[Occupancy measure]
    Given a policy $\pi$, we define the occupancy measure of $\pi$ as 
    $$
        \mu_{\pi}(x, a) = P_X(x) \pi(a \mid x).
    $$
    Note that occupancy measure is independent of bandit instance as we assume the same context distribution.
\end{defn}

\begin{defn}[Learning algorithm]
    We denote a learning algorithm by $L = (L^{(1)}, L^{(2)})$, where $L^{(1)}$ is an online learning algorithm that is a deterministic mapping from history $\gH_t = (X_{\tau}, A_{\tau}, Y_{\tau})_{\tau = 1}^{t-1}$ to a policy in $\Pi^{(1)}$. Here, $L^{(2)}$ is an offline learning algorithm that maps $\gH_{T+1}$ to a policy $\hat \pi \in \Pi^{(2)}$. Note that $L^{(i)}$ can depend on $f^{(i)}$ and $\Pi^{(i)}$ for each $i \in \{1, 2\}$ as they are known knowledge. We denote the set of all such algorithms by $\gL$.
\end{defn}

For some instance set $\gS$, we study the following minimax multi-objective optimization problem:
\begin{equation}
    \inf_{L \in \gL} \sup_{P \in \gP} \left(\E[\CR], \E[\SR(\hat\pi)]\right).
\end{equation}

In order to show a more restrictive lower bound for the above multi-objective problem, we need the instance set $\gS$ to be adequately rich. Theorem \ref{thm:lower_bound_pi_f} provides general conditions on $\gS$ for the lower bound to hold. %, under which we may show that $\inf_{L} \sup_{S}\sqrt{\E \left[\Reg_1 \right]} \E \left[\Reg_2 \right] / T_2 = \Omega(1)$. 
% \kwz{I'm trying to understand reasoning behind when you have an expectation around Reg1 and Reg2 vs you when don't have expectations like in in display (1)). Also in the intro there is no expectation around Reg1.}
% \ziping{I should prob. add expectation in (1) as well}

% \begin{thm}
% \label{thm:lower_bound_pi_f}
%     Assume the problem instance set $\gS$ is sufficiently large to ensure the existence of an instance $\mS = (S^{(1)}, S^{(2)})$ such that for all $\epsilon \in [0, 1/4]$, we can find some $\bar{\mS} = (\bar{S}^{(1)}, \bar{S}^{(2)}) \in \gS(\mS)$ satisfying the following conditions for some $(x_{\star}, a_{\star}) \in \gX \times \gA$:
%     \begin{enumerate}
%         \item $\mu_{\pi_{S^{(1)}}^{\star}}(x_{\star}, a_{\star}) = \mu_{\pi_{\bar{S}^{(1)}}^{\star}}(x_{\star}, a_{\star}) = 0$ and $\min\{\SR_{S^{(1)}}(\pi), \SR_{\bar{S}^{(1)}}(\pi)\} \geq c_1 \mu_{\pi}(x_{\star}, a_{\star})$ for all $\pi \in \Pi^{(1)}$;
%         \item $\mu_{\pi^{\star}_{S^{(2)}}}(x_{\star}, a_{\star}) - \mu_{{\pi}^{\star}_{\bar{S}^{(2)}}}(x_{\star}, a_{\star}) = c_2 > 0$;
%         \item $\operatorname{SR}_{S^{(2)}}(\pi) \geq \epsilon(\mu_{\pi^{\star}_{S^{(2)}}}(x_{\star}, a_{\star}) - \mu_{\pi}(x_{\star}, a_{\star}))/2$ for all $\pi \in \Pi^{(2)}$;
%         \item $\operatorname{SR}_{\bar{S}^{(2)}}(\pi) \geq \epsilon(\mu_{\pi}(x_{\star}, a_{\star}) - \mu_{\pi^{\star}_{\bar{S}^{(2)}}}(x_{\star}, a_{\star}))/2$ for all $\pi \in \Pi^{(2)}$;
%         % \item $\mu_{\pi^\star(S^{(2)})}^{(2)}(x, a) \geq C_3 > 0$;
%         \item $D_{\operatorname{KL}}(P(\cdot \mid x_{\star}, a_{\star}) \mid \bar{P}(\cdot \mid x_{\star}, a_{\star})) \leq \epsilon^2$,
%     \end{enumerate}
%     where $c_1, c_2 > 0$ are some constant and $(x_{\star}, a_{\star}) \in \gX \times \gA$ is some context-action pair.
%     Then we have the following lower bound:
%     \begin{equation}
%         \inf_{L \in \gL_2} \sup_{\mS \in \gS} \sqrt{\E \left[\Reg_1 \right]} \E \left[\Reg_2 \right] / T_2  = \Omega\left(c_1 c_2\right). \label{equ:thm1}
%     \end{equation}
% \end{thm}


\begin{thm}
\label{thm:lower_bound_pi_f}
    Let the policy classes and reward mappings be $\Pi^{(1)}, f^{(1)}$, and $\Pi^{(2)}, f^{(2)}$, for tasks 1 and 2, respectively. Assume the outcome distribution set is sufficiently rich to ensure the existence of an instance $P \in \gP$ such that for any $\epsilon \in [0, 1/4]$, we can find some $\bar P \in \gP$ satisfying the following conditions for some $(x_{\star}, a_{\star})$:
    \begin{enumerate}
        \item $\mu_{\pi_{1}^{\star}}(x_{\star}, a_{\star}) = \mu_{\pi_{2}^{\star}}(x_{\star}, a_{\star}) = 0$;
        \item $\exists \pi \in \Pi^{(2)}, \mu_{\pi}(x_{\star}, a_{\star}) > 0$;
        \item ${\SR}(\pi) = \epsilon(\mu_{\pi}(x_{\star}, a_{\star}) - \mu_{{\pi}_2^{\star}}(x_{\star}, a_{\star}))/2, \forall  \pi \in \Pi^{(2)}$;
        \item $D_{\operatorname{KL}}(P(\cdot | x_{\star}, a_{\star}) \mid \bar{P}(\cdot | x_{\star}, a_{\star})) \leq \epsilon^2$;
        \item $\E_{\bar{P}}[f^{(2)}(Y_t) \mid X_{t} = x_{\star}, A_t = a_{\star}]$ = $\E_{P}[f^{(2)}(Y_t) \mid X_{t} = x_{\star}, A_t = a_{\star}] + \epsilon
        $
    \end{enumerate}
    
    % for all $\epsilon \in [0, 1/4]$, we can find some $\bar{\mS} = (\bar{P}, \Pi^{(1)}, f^{(1)}, \Pi^{(2)}, f^{(2)}) \in \gS$ satisfying the following conditions for some $(x_{\star}, a_{\star}) \in \gX \times \gA$:
    % \begin{enumerate}
    %     \item $\mu_{\pi_{1}^{\star}}(x_{\star}, a_{\star}) = \mu_{\bar{\pi}_{1}^{\star}}(x_{\star}, a_{\star}) = 0$;
    %     \item $\mu_{\pi^{\star}_{2}}(x_{\star}, a_{\star}) - \mu_{{\bar\pi}^{\star}_{2}}(x_{\star}, a_{\star}) > 0$;
    %     \item $\SR(\pi) \geq \epsilon(\mu_{\pi^{\star}_{2}}(x_{\star}, a_{\star}) - \mu_{\pi}(x_{\star}, a_{\star}))/2, \forall \pi \in \Pi^{(2)}$;
    %     \item $\overline{\SR}(\pi) \geq \epsilon(\mu_{\pi}(x_{\star}, a_{\star}) - \mu_{\bar{\pi}_2^{\star}}(x_{\star}, a_{\star}))/2, \forall  \pi \in \Pi^{(2)}$;
    %     % \item $\mu_{\pi^\star(S^{(2)})}^{(2)}(x, a) \geq C_3 > 0$;
    %     \item $D_{\operatorname{KL}}(P(\cdot \mid x_{\star}, a_{\star}) \mid \bar{P}(\cdot \mid x_{\star}, a_{\star})) \leq \epsilon^2$.
    % \end{enumerate}
    Then we have the following lower bound:
    \begin{equation}
        \inf_{L \in \gL} \sup_{P \in \gP} \sqrt{\E \left[\CR \right]} \E \left[\SR \right]  = \Omega\left(1\right). \label{equ:thm1}
    \end{equation}
\end{thm}

% \paragraph{Discussion of Theorem \ref{thm:lower_bound_pi_f}.} Discuss what each condition means here.

% \ziping{Should mention that we are interested in the rate in $T_1$ and $T_2$ only}

\paragraph{Discussion of Theorem \ref{thm:lower_bound_pi_f}.} A significant difference between (\ref{equ:thm1}) and the existing result in (\ref{equ:existing_lower}) is that the rate for $\E[\CR_1]$ in (\ref{equ:existing_lower}) becomes square root. To understand the legitimacy of the new square root, we note that in order to optimize the $\CR_2$'s rate in $T_1$, one could adopt a purely random exploration in the first task, which gives the $\E[\CR_2 / T_2] = \tilde{\Theta}(1/\sqrt{T_1})$. This is the regular error rate (w.r.t. sample size) one would expect for estimating a parametric model.


We further explain the intuitions of Condition2 1-6. For sufficiently large $T_1$, a no-regret online algorithm tends to converge to the optimal policy (assuming there exists a unique one and there is a lower bounded suboptimality gap). This dataset collected from online learning of the first task may not be sufficient for the goal of offline policy optimization for the second task, when $\max_{x, a}\mu_{\pi^\star_{S^{(2)}}}(x, a) / \mu_{\pi^\star_{S^{(1)}}}(x, a) = \infty$ (guaranteed by Condition 2). This connects closely to the offline learning literature, where it has been shown that offline learning is fundamentally hard if the single-policy concentrability is unbounded \citep{chen2019information}. Single-policy concentrability is the ratio between the occupancy measures of the behavior policy that collects the offline dataset and the optimal policy. Condition 2 guarantees that it incurs regret whenever $(x_{\star}, a_{\star})$ is visited in the first task, and Condition 3, 4 and 5 guarantee that it is necessary to visit $(x_{\star}, a_{\star})$ to distinguish between $S^{(2)}$ and $\bar{S}^{(2)}$, which creates the tension between the regrets of two tasks. 



%The induced reward functions are reported in Table \ref{tab:reward_table}.

\subsection{Case studies on Theorem \ref{thm:lower_bound_pi_f} application}
\label{sec:case-study}
In this section, we explore two case studies with potential practical interests to demonstrate how the  conditions specified in Theorem \ref{thm:lower_bound_pi_f} can be satisfied by including potential changes in $\Pi$ and $f$. To ease the demonstration, we consider uniform distribution $P_X$ over context space $\gX$. The first case is a two-task contextual bandit problem with $\gA = \{a_1, a_2\}$ and $\gX = \{x_1, x_2\}$. The second case is an multi-armed problem with $\gA = \{a_1, a_2\}$.

\paragraph{Case I: adding a new feature.} In real-world implementations, some features that were excluded from the input may be added back in the later tasks. To conceptualize this, we consider $\Pi^{(1)}$ as the set of policies where decision-making is independent of current features, formalized as $\Pi^{(1)} = \{\pi: \pi(\cdot \mid x_1) = \pi(\cdot \mid x_2), \text{for all } x_1, x_2 \in \gX\}$. Conversely, let $\Pi^{(2)}$ encompass all possible policies. The mean reward function $R$ and $\bar R$ induced by outcome distribution $P$ and $\bar{P}$ is given by Table \ref{tab:case1}. For all positive $\epsilon$, $\pi^\star_{S^{(1)}}(a_1 \mid \cdot) \equiv 1$.  Any policy with a non-zero occupancy measure on $(x_2, a_2)$ will have the same occupancy measure on $(x_1, a_2)$, leading to simple regret of $1/2 - \epsilon$. However, the optimal policies of $S^{(2)}$ and $\bar{S}^{(2)}$ disagree on $x_2$. To distinguish $\bar{S}$ from $S$, the algorithm is forced to visit $(x_2, a_2)$ in the first task. The conditions in Theorem \ref{thm:lower_bound_pi_f} is satisfied with $c_1 = 1/2 - \epsilon$ and $c_2 = 1/2$.


\begin{table}[ht]
% \small
% \begin{subtable}%{0.45\textwidth}
% \caption{Reward tables for different case studies}
\centering
    \begin{minipage}[c]{0.54\textwidth}
    \centering
    \caption{Case I: adding a new feature}
    \label{tab:case1}
    \begin{tabular}[t]{c|c|c|c || c|c|c|c}
        $R$ & $x_1$ & $x_2$ & $\bar{x}$ & $\bar{R}$ & $x_1$ & $x_2$ & $\bar{x}$ \\
        \hline
        $a_1$  & 1+$\epsilon$ & 1-$\epsilon$ & 1 & $a_1$ & 1+$\epsilon$ & 1-$\epsilon$ & 1  \\
        $a_2$ & 0 & 1 & 0.5 & $a_2$ & 2$\epsilon$ & 1-2$\epsilon$ & 0.5
    \end{tabular}
    \end{minipage}
    % \begin{minipage}[c]{0.31\textwidth}
    % \centering
    % \caption{Case II}
    % \label{tab:case2}
    % \begin{tabular}[t]{c|c|c || c|c|c}
    %     $R$ & $x_1$ & $x_2$ & $\bar R$ & $x_1$ & $x_2$ \\
    %     \hline
    %     $a_1$  & 1 & 0 & $a_1$ & 1 & $\epsilon$ \\
    %     $a_2$ & $\epsilon/2$ & 1 & $a_2$ & $\epsilon/2$ & 1
    % \end{tabular}
    % \end{minipage}
    \begin{minipage}[c]{0.45\textwidth}
    \centering
    \caption{Case II: change of reward function}
    \label{tab:case3}
    \centering
    \begin{tabular}[t]{c|c|c || c|c}
         & $R^{(1)}$ & $R^{(2)}$  & $\bar{R}^{(1)}$ & $\bar R^{(2)}$ \\
        \hline
        $a_1$  & 1 & 0.5  & 1 & 0.5\\
        $a_2$  & 0.8 & 0.5-$\epsilon$/2  & 0.8 & 0.5+$\epsilon$/2
    \end{tabular}
    
    \end{minipage}
    
% \caption{Reward table for different case studies.}
    \label{tab:reward_table}
\end{table}

% \begin{table}[ht]
% % \begin{subtable}%{0.45\textwidth}
% \caption{Reward tables for different case studies}
%     \begin{minipage}[c]{0.34\textwidth}
%     \caption{Case I}
%     \label{tab:case1}
%     \begin{tabular}[t]{c|c|c}
%         $R$ & $x_1$ & $x_2$ \\
%         \hline
%         $a_1$  & 1-$\epsilon$ & 1-$\epsilon$  \\
%         $a_2$ & 0 & 1 \\ 
%         \hline\hline
%         \vspace{-3.5mm} \\
%         $\bar{R}$ & $x_1$ & $x_2$ \\
%         \hline
%         $a_1$ & 1-$\epsilon$ & 1-$\epsilon$ \\
%         $a_2$ & 0 & 1-2$\epsilon$
%     \end{tabular}
%     \end{minipage}
%     \begin{minipage}[c]{0.31\textwidth}
%     \centering
%     \caption{Case II}
%     \label{tab:case2}
%     \begin{tabular}[t]{c|c|c || c|c|c}
%         $R$ & $x_1$ & $x_2$ \\
%         \hline
%         $a_1$  & 1 & 0\\
%         $a_2$ & $\epsilon/2$ & 1 \\
%         \
%         $\bar R$ & $x_1$ & $x_2$\\
%         \hline
%          $a_1$ & 1 & $\epsilon$ \\
%          & $a_2$ & $\epsilon/2$ 
%     \end{tabular}
%     \end{minipage}
%     \begin{minipage}[c]{0.3\textwidth}
%     \caption{Case III}
%     \label{tab:case3}
%     \centering
%     \begin{tabular}[t]{c|c|c || c|c}
%          & $R^{(1)}$ & $R^{(2)}$  & $\bar{R}^{(1)}$ & $\bar R^{(2)}$ \\
%         \hline
%         $a_1$  & 1 & 0.5  & 1 & 0.5\\
%         $a_2$  & 0.8 & 0.5-$\epsilon$/2  & 0.8 & 0.5+$\epsilon$/2
%     \end{tabular}
    
%     \end{minipage}
    
% % \caption{Reward table for different case studies.}
%     \label{tab:reward_table}
% \end{table}

% \paragraph{Case II: removing an old feature.} Some features may have to be removed over a sequence of implementations due to potential ethic issues. For this consideration, we let $\Pi^{(1)}$ be the set of all policies and $\Pi^{(2)} = \{\pi: \pi(\cdot \mid x_1) = \pi(\cdot \mid x_2), \text{for all } x_1, x_2 \in \gX\}$. Table \ref{tab:case2} demonstrates a pair of instances, where the optimal policies for the first task always select action $a_1$ under context $x_1$ and action $a_2$ under context $x_2$. Any non-zero occupancy measure on $(x_2, a_1)$ induces an instant regret of at least $1-\epsilon$ for both $S^{(1)}$ and $\bar{S}^{(1)}$. Nevertheless, the optimal actions for $S^{(2)}$ and $\bar{S}^{(2)}$ are $a_2$ and $a_1$, respectively, and it requires the first task to have a coverage on $(x_2, a_1)$ to distinguish between $S$ and $\bar{S}$. The conditions in Theorem \ref{thm:lower_bound_pi_f} is satisfied with $c_1 = 1-\epsilon$ and $c_2 = 1/2$.

\paragraph{Case II: change of reward function.} The reward functions may change over a sequence of implementations. For instance, let outcome $Y_{i, t} = (R_{i, t}, W_{i, t})$, where $R_{i, t}$ is the primary outcome we intend to maximize and $W_{i, t}$ is a potential side effects. In the first implementation, we aim at maximizing the primary outcome $R_{i, t}$ with reward function $f^{(1)}(Y_{1, t}) = R_{1, t}$. However, the domain expert may realize that $W_{i, t}$ is a strong side effect, which should be controlled in the second task, and thus, they set the reward function as $f^{(2)}(Y_{2, t}) = R_{2, t} - \alpha W_{2, t}$. With this motivation, we construct  a pair of multi-armed bandit instances with no context. In Table \ref{tab:case3}, we demonstrate the mean reward of different arms under different combinations of $f^{(1)}$, $f^{(2)}$, $P$ and $\bar P$. In the first task, a regret of $0.2$ is incurred whenever $a_2$ is pulled, while a sufficient pulling of $a_2$ is necessary to distinguish $P$ from $\bar{P}$. It can be verified that the conditions in Theorem \ref{thm:lower_bound_pi_f} holds with $c_1 = 0.2$ and $c_2 = 1$.

A detailed verification of how the two cases satisfy the conditions in Theorem \ref{thm:lower_bound_pi_f} is deferred to Appendix \ref{app:case_study}.

\subsection{Optimal level of exploration}

As implied by Theorem \ref{thm:lower_bound_pi_f}, any algorithm that achieves an optimal rate in $\Reg_1$ is suboptimal in $\Reg_2$. To trade-off between the two goals, the algorithm needs to employ additional exploration in the first task. In this section, we characterize the optimal level of additional exploration in different regimes of $T_1$ and $T_2$. Since we primarily focus on the role of horizons, we omit the dependence on $|\gX|$ and $|\gA|$ throughout the discussions on this section. 

Recall that our primary goal is to minimize global regret, that is the sum of cumulative regrets of two tasks. Proposition \ref{prop:lower_bound_sum} suggests a minimax lower bound for the sum of cumulative regrets of two tasks that is the maximum of three terms--$T_2/\sqrt{T_1}, T_2^{2/3}$ and $\sqrt{T_1}$. The $T_2 / \sqrt{T_1}$ term corresponds to the case, where $\E[\Reg_2]$ dominates $\E[\Reg_1]$, and the minimax rate of simple regret in the second for any dataset collected during the first task is $T_2 / \sqrt{T_1}$. The second term corresponds to the rate characterized by Theorem \ref{thm:lower_bound_pi_f}. The last term of $\sqrt{T_1}$ is the minimax rate of the first task regret minimization. This corresponds to the case when $\E[\Reg_1]$ dominates $\E[\Reg_2]$.
%\ziping{talk about which term domains}
%\sam{explain how Thm 1 suggests this lower bound...}
\begin{prop}
\label{prop:lower_bound_sum}
Following the same conditions on the instance set $\gS$ as in Theorem \ref{thm:lower_bound_pi_f}, the following minimax lower bound holds
\begin{equation}
    \inf_{L_2 \in \gL} \sup_{S \in \gS} \E[\Reg_1 + \Reg_2] = \Omega\left( \max\left\{\frac{T_2}{\sqrt{T_1}}, T_2^{2/3}, \sqrt{T_1}\right\}\right) \label{equ:three_lower}
\end{equation}
\end{prop}


We show that a simple algorithm that mixes a minimax-optimal online learning algorithm with a purely random exploration has upper bounded global regret that matches the lower bound in Theorem \ref{thm:lower_bound_pi_f} up to a factor of $|\gX| |\gA|$. This also allows us to achieve any point on the Pareto frontier up to a factor of $|\gX| |\gA|$. The parameter $\alpha$ controls the level of additional exploration in the first task. 
\begin{thm}
\label{thm:upper_bound}
    Let $L_0$ be an online learning algorithm with a regret bound of $\mathcal{O}(\sqrt{|\gX||\gA|T_1})$ on the first task. Let the algorithm for the first task be $L_{\alpha}(\tau) = (1-\alpha) L_0(\tau) + \alpha \pi_0$, where $\tau$ is any past observations and $\pi_0$ is the uniform random policy. For any choice of $\alpha \in [{|\gX| |\gA|}/{\sqrt{T_1}}, 1]$, there exist offline-learning algorithm for the second task such that
    \begin{equation}
        \E[\Reg_1] = \gO\left(\alpha T_1 \right), \quad \E[\Reg_2/T_2] = \gO\left(\sqrt{\frac{(|\gX| |\gA|)^2}{\alpha T_1}} \right). \label{equ:upper_bound}
    \end{equation}
\end{thm}


By tuning the exploration rate $\alpha$, we are able to match the minimax lower bound provided in (\ref{equ:three_lower}). In short, there are three regimes of $(T_1, T_2)$, for which we should choose different levels of exploration rate $\alpha$ to balance $\E[\Reg_1]$ and $\E[\Reg_2]$. The regime one is when $T_1 \leq T_2^{2/3}$, where the first task is too short compared to the second task, and the algorithm should employ pure exploration in the first task ($\alpha = 1$). This regime leads to a global regret of $\gO({T_2}/{\sqrt{T_1}})$. In an intermediate regime with $T_2^{2/3} < T_1 \leq T_2^{4/3}$, the algorithm should employ additional exploration compared to these that achieve a minimax optimal rate in a single task. Theorem \ref{thm:upper_bound} suggests an additional exploration rate of $\alpha = T_2^{2/3} / T_1$ and a global regret bound of $\gO(T_2^{2/3})$. Note that under a special case of $T_1 = T_2$, the rate of $\alpha = T_1^{-1/3}$ indicates a regret bound of $\gO(T_1^{2/3})$ in the first task. The third regime is $T_1 > T_2^{4/3}$, where one should employ $\alpha = 0$, meaning that no excess exploration is needed and the agent in the first task can minimize the local regret as much as possible. In this regime, the local regret in the first task could achieve the minimax optimal rate of $\sqrt{T_1}$. 

It is often in real-world applications that $T_2$ is pre-determined and the researcher could decide how many samples to collect in the first task to ensure a good learning in the second one. For instance, in an inventory management context \citep{madeka2022deep}, it is determined by the engineering team that how long a learned policy should be deployed for the second task. In such cases, our theory indicates that one should choose $T_1 > T_2^{4/3}$, so a greedy local regret minimization for the first task is justified.

